Spatial Cross-Attention Improves Self-Supervised Visual Representation Learning

Unsupervised representation learning methods like SwAV are proved to be effective in learning visual semantics of a target dataset. The main idea behind these methods is that different views of a same image represent the same semantics. In this paper, we further introduce an add-on module to facilitate the injection of the knowledge accounting for spatial cross correlations among the samples. This in turn results in distilling intra-class information including feature level locations and cross similarities between same-class instances. The proposed add-on can be added to existing methods such as the SwAV. We can later remove the add-on module for inference without any modification of the learned weights. Through an extensive set of empirical evaluations, we verify that our method yields an improved performance in detecting the class activation maps, top-1 classification accuracy, and down-stream tasks such as object detection, with different configuration settings.

==> Sections/4_Related_Works.tex <==
\section{Related Work}
\mehdi{\textbf{Coming Soon}}
\begin{comment}
The dramatic performance of deep neural networks is directly proportional to the amount of training data available. The more sophisticated architectures, trained on large scale datasets continue to set new state-of-the-art (SOTA) records. However, collection, and annotation of large datasets are timely matters.
To overcome the costly and laborious data annotation, many self-supervised/unsupervised representation learning methods were developed to extract the visual distillate of the large-scale images without the burden of labeling them. The distillates are meant to be preserving useful visual information when representing the images in a downstream task. These visual features may be chosen to be task specific, i.e., they can be optimized to preform better in specific task, e.g., classification, detection, segmentation, etc, or might be task-general.  One popular solution to learn the visual representations is to train the network to solve one or multiple pretext tasks on the unlabeled dataset thereby introducing objective functions which must be optimized through gradient descent. Several pretext tasks have been designed so far for self representation learning, which some common ones include, solving a jigsaw puzzle\cite{noroozi2016unsupervised}, gray scale image colorization \cite{zhang2016colorful}, and automatic image inpainting\cite{pathak2016context}. 

A breakthrough for designing pretext tasks occurred by the introduction of contrastive learning\cite{Wu_2018_CVPR} and infoNCE loss\cite{oord2018representation,henaff2019data}. The contrastive representation learning idea is to train a network that is able to discriminate between the images in the dataset thereby minimizing the similarity between their representation features through infoNCE loss. Later \cite{Misra_2020_CVPR} and \cite{cvpr19unsupervised} reasoned that useful image representations must be invariant under semantic preserving image transformations. This observation formed the foundation of many newer SOTA algorithms in this filed. To comply with this observation these algorithms try to discriminate images against each other within a dataset by minimizing their cosine similarity and at the same time force the representations of the transformed counter parts of the same image to be close in terms of their normalized inner product\cite{he2019moco, chen2020mocov2,caron2020unsupervised,grill2020bootstrap}.

Some methods use the infoNCE to discriminate the feature vectors and then use Kmeans to cluster the feature vectors\cite{li2020prototypical, van2020learning,zhuang2019local}. In this paper however, unlike these algorithms we tend to cluster the representation space on the fly.
Similar to the work of He, et al.\cite{he2019moco}, we use a momentum-encoder architecture to discriminate the images within the dataset. We utilize the infoNCE loss as a discriminator, meaning while it pulls similar image representations together, it pushes away representations that do not belong to the same image. We propose via this setup, to cluster the dataset using both the encoder and momentum-encoder, simultaneously. Each of the representations that are clustered by both of these architectures, belong to a cluster through a probability distribution. We optimize the weights of the encoder architecture by minimizing the cross entropy between the probability distributions of each cluster generator, i.e., the encoder and the momentum-encoder. The momentum-encoder weights are updated via momentum updates as in \cite{he2019moco,chen2020mocov2,grill2020bootstrap}. Assigning a random variable to each feature vector, we manage to maximize the representations' entropy, to insure that the feature vectors are uniformly distributed over the clusters. We call this part of the algorithm Bi-Moco, since it uses Moco twice on the same dataset, thereby clustering the same dataset by two architectures. We show that this setup, under the common linear-head protocol, improves Moco's performance by approximately $2\%$ on the Imagenet dataset. We then extend the idea of Bi-Moco to Multi-Moco by modifying the multi-crop augmentation technique proposed by \cite{caron2020unsupervised, zhuang2019local,asano2019self}. Later, we also introduce DeepAugment \cite{hendrycks2020faces}, to the self-supervised learning community. DeepAugment, is an augmentation technique that generates transformed images by distorting the weight of a pre-trained image-to-image network such as super-resolution auto-encoder, randomly. We show that Deepaugment, along with mixture of other transformations is quite helpful and improves the performance of our algorithm by another $5\%$.
We validate our contributions on a standard Imagenet dataset following the linear head protocol. We show that our algorithm achieves the SOTA performance when trained on Imagenet with no labels for 200 epochs.
\end{comment}


==> Sections/Experiments/EX_Cifar10.tex <==
\subsection{CIFAR Experiments}
In this section we experiment the functionality of our proposed add-on on the Cifar-10 \cite{krizhevsky2009learning} dataset. We use a version of Resnet-18 as the backbone for our experiment tailored for a the Cifar-10 small $32\times 32$ input image size \cite{Idelbayev18a}.  
In our experiments, we remove the \texttt{Gaussian blur} augmentation and will reduce the strength of \texttt{ColorJitter} to $1/4$. We use $K=30$ as the number of prototypes for the SwAV core engine. We use same cosine scheduler and temperature values as before. The batch size for all experiments is 256. We fine-tuned SwAV baseline on Cifar-10 with $\texttt{lr} = .6$ and final learning rate of $.0006$. We also use a 10 epoch warmup with initial learning rate of $.3$. For our method the best hyper-parameters are tuned as before except the learning rate is set to 2.6 with initial learning rate of .3 and final learning rate of .0026. 


==> Sections/Experiments/EX_Key_point.tex <==
\subsection{COCO Key-Point Detection}
The key-point version of Mask R-CNN with Resnet-50 base and FPN backbone (R-50-FPN),
is fine-tuned on COCO \texttt{train2017}
and evaluated on \texttt{val2017}. for $180k$ iterations.

\begin{table}[bth!]
\footnotesize
\centering
\begin{tabular}{c|c}
   &COCO keypoint detection\\

\hline
pre-train&  
\begin{tabular}{ccc} $\textrm{AP}^{\textrm{kp}}$ & $\textrm{AP}_{50}^{\textrm{kp}}$ & $\textrm{AP}_{75}^{\textrm{kp}}$ \end{tabular}\\
\hline
scatch&  
\begin{tabular}{ccc} 65.9& 86.5 &71.7\end{tabular}\\
\hline
Imagenet-1K-pretraining&  
\begin{tabular}{ccc} 65.8& 86.9& 71.9 \end{tabular}\\
\hline

SwAV+repr&  
\begin{tabular}{ccc} 66.2 &87.1 & 72.6 \end{tabular}\\
\hline

%sults for keypoints_coco_2017_val in csv format:
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: Task: bbox
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: AP,AP50,AP75,APs,APm,APl
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: 55.8426,83.9362,61.2932,38.7339,63.2845,72.2228
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: Task: keypoints
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: AP,AP50,AP75,APm,APl
% [32m[05/19 17:47:08 d2.evaluation.testing]: [0mcopypaste: 66.2994,86.9981,72.5261,62.2601,74.0564
 ours&  
\begin{tabular}{ccc} 66.2 & 86.9 & 72.5 \end{tabular}\\
\hline

\end{tabular}
% \vspace{.2cm}
\caption{\footnotesize{Transfer Learning. COCO key point detection.}}
\label{tab:key_point_detection}
\end{table}


==> Sections/Experiments/EX_Other_Datasets.tex <==
%-------------------------------------------Other Datasets Results -----------------------------------

\subsubsection{Other Datasets Results}
If a good representation is learned during the pre-training, then it should generalize well with a little fine-tuning effort. To evaluate the quality of the learned features, we transfer the representations learned from unsupervised training of Resnet-50 on Imagenet-1K to other datasets. Particularly, we Freeze the Resnet-50 body weights and we train a linear head on VOC07\cite{everingham2010pascal}, Places205\cite{zhou2014learning}, and COCO\cite{lin2014microsoft} datasets following the training and evaluation setup in \cite{zhang2017split}. Similar to \cite{Goyal_2019_ICCV}, we use SGD optimizer, batch size of 256, and learning rate of .01 with a decay factor of 10 after each $40k$ iterations. After that we train on \textrm{train split} for $140k$ iterations. The accuracy on the \textrm{val split} can be seen in Table \ref{table_classification_linear}.  
\begin{table*}[h]
\centering
\begin{tabular}{llcccccc}
 \multicolumn{8}{c}{Classification transfer learning to other datastes under linear head protocol} \\
 \hline
 Method                             & Architecture   & Top-1 acc & Epochs &COCO2014& VOC07&Places205\\
 \hline
 MOCO\cite{he2019moco}              &Res-50 x 1      &        &200 &   &   &   \\
 
 SimCLR\cite{chen2020simple}        &Res-50 x 1      &        &200&   &   &\\
 CPC-v2\cite{henaff2019data}        &Res-50 x 1      &        &-          &-&   &   &\\        
 MOCO-v2\cite{chen2020mocov2}       &Res-50 x 1      &        &200&   &   &\\
 SwAV\cite{caron2020unsupervised}   &Res-50 x 1      &        &200&   &   &\\
 InfoMin Aug.\cite{tian2020makes}   &Res-50 x 1      &        &200&   &   &\\
\hline
 Bi-Moco(ours)                      &Res-50 x 1       &        &200&   &   &\\
\hline
 Bi-Moco + DeepAugment (ours)       &Res-50 x 1       &        &200&   &   &\\
\hline

 XMoco(ours)                        &Res-50 x 1       &        &200&   &   &\\
\hline
\\
\end{tabular}
\caption{Classification transfer learning to other datastes under linear head protocol}
\label{table_classification_linear}
\end{table*}


==> Sections/Key_Points.tex <==

\section{Key Sentences we used in the related works}
\begin{itemize}
\item In this paper we try to argue that it is important that the model knows where to look in the image for the most informative features.
\item Incorporate intra-class information in the learning process thereby selecting images in the same cluster in an unsupervised manner
\item Distilling cross correlation information between same clustered images and constitute an explanation map via creating an attention-like mask on top of each feature-map.
\item self supervised classifying of the explanation maps.
\end{itemize}
\subsection{Injecting Extra Knowledge to the Model}
\begin{itemize}
\item Find images with close enough representations and consider them to be in the same class.
\item Search for similar features in the images' feature maps.
\item Via searching for the most correlated features across the same-class feature-map grids, we localize and emboss the areas that carry information about the intersecting features within positive images. 
\item Explanation maps are constituted thereby embossing the commonalities and muting the other parts across the positive feature maps.
\item Explanation maps are then trained thereby feeding the add-on network with labels gathered by clustering the memory.
\item We try to increase the output confidence score by feeding the most important parts (explanation maps) to the network.
\item Simultaneously, and on the contrary, we try to hold up the prediction score as only a part of the features is fed to the classifier head. We expect that this would decrease the average drop of the network.

\end{itemize}


==> styles/Commands.tex <==




